Forest: Structural Code Editing with Multiple Cursors

Software developers frequently refactor code. Often, a single logical refactoring change involves changing multiple related components in a source base such as renaming each occurrence of a variable or function. While many code editors can perform such common and generic refactorings, they do not support more complex refactorings or those that are specific to a given code base. For those, as a flexible - albeit less interactive - alternative, developers can write refactoring scripts that can implement arbitrarily complex logic by manipulating the program's tree representation. In this work, we present Forest, a structural code editor that aims to bridge the gap between the interactiveness of code editors and the expressiveness of refactoring scripts. While structural editors have occupied a niche as general code editors, the key insight of this work is that they enable a novel structural multi-cursor design that allows Forest to reach a similar expressiveness as refactoring scripts; Forest allows to perform a single action simultaneously in multiple program locations and thus support complex refactorings. To support interactivity, Forest provides features typical for text code editors such as writing and displaying the program through its textual representation. Our evaluation demonstrates that Forest allows performing edits similar to those from refactoring scripts, while still being interactive. We attempted to perform edits from 48 real-world refactoring scripts using Forest and found that 11 were possible, while another 17 would be possible with added features. We believe that a multi-cursor setting plays to the strengths of structural editing, since it benefits from reliable and expressive commands. Our results suggest that multi-cursor structural editors could be practical for performing small-scale specialized refactorings.

==> examples/cpojer-js-codemod-jest-arrow-0.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^describe("describe", function () {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  it("should be happy", function () {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    console.log("actually forwards body");^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  });^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  it("should leave arrow functions", () => {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  describe("nested describe", function () {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    xit("disabled still counts", function () {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    xdescribe("disabled describe", function () {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  });^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^function containsit() {}^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^containsit(function () {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      
    \end{flushleft}
  

==> examples/cpojer-js-codemod-jest-arrow-1.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^describe("describe", function () {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ^\strut\UseVerb{Verb}\SaveVerb{Verb}^it("should be happy", function () {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    console.log("actually forwards body");^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  })^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  it("should leave arrow functions", () => {});^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  describe("nested describe", function () {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    ^\strut\UseVerb{Verb}\SaveVerb{Verb}^xit("disabled still counts", function () {})^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    ^\strut\UseVerb{Verb}\SaveVerb{Verb}^xdescribe("disabled describe", function () {})^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  });^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^});^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^function containsit() {}^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^containsit(function () {});^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      Use structural search UI (not shown) to find calls with callee names matching a regular expression and having a function expression as the second argument\\
\keys{\shift+s}\hspace{2mm}\keys{\arrowkeydown}
    \end{flushleft}
  

==> examples/cpojer-js-codemod-jest-arrow-2.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^describe("describe", function () {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  it^\strut\UseVerb{Verb}\SaveVerb{Verb}^("should be happy", () => {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    console.log("actually forwards body");^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  })^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  it("should leave arrow functions", () => {});^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  describe("nested describe", function () {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    xit^\strut\UseVerb{Verb}\SaveVerb{Verb}^("disabled still counts", () => {})^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    xdescribe^\strut\UseVerb{Verb}\SaveVerb{Verb}^("disabled describe", () => {})^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  });^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^});^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^function containsit() {}^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^containsit(function () {});^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{\{}\hspace{2mm}\keys{\}}\hspace{2mm}\keys{c}\hspace{2mm}\keys{\arrowkeyup}\hspace{2mm}\keys{i}\\
Type \SaveVerb{Verb}^()=>{},^\adjustbox{bgcolor={HTML}{F2F2F2}}{\strut\UseVerb{Verb}}\\
\keys{\esc}\hspace{2mm}\keys{\{}\hspace{2mm}\keys{\}}\hspace{2mm}\keys{p}\hspace{2mm}\keys{\shift+\arrowkeyright}\hspace{2mm}\keys{\SPACE}\hspace{2mm}\keys{d}
    \end{flushleft}
  

==> examples/cpojer-js-codemod-jest-arrow-3.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^describe("describe", function () {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  it("should be happy", () => {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    console.log("actually forwards body");^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  });^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  it("should leave arrow functions", () => {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  describe("nested describe", function () {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    xit("disabled still counts", () => {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    xdescribe("disabled describe", () => {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  });^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^function containsit() {}^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^containsit(function () {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{)}\hspace{2mm}\keys{)}\hspace{2mm}\keys{)}\hspace{2mm}\keys{\arrowkeyup}\hspace{2mm}\keys{\arrowkeyup}\hspace{2mm}\keys{\shift+s}\hspace{2mm}\keys{f}
    \end{flushleft}
  

==> examples/cpojer-js-codemod-jest-arrow-4.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^describe("describe", function () {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  it("should be happy", () => {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    console.log("actually forwards body");^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  });^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  it("should leave arrow functions", () => {});^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ^\strut\UseVerb{Verb}\SaveVerb{Verb}^describe("nested describe", function () {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    xit("disabled still counts", () => {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    xdescribe("disabled describe", () => {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  })^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^});^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^function containsit() {}^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^containsit(function () {});^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      Use structural search UI (not shown) to find calls with callee names matching a regular expression and having a function expression as the second argument\\
\keys{\shift+s}\hspace{2mm}\keys{\arrowkeydown}
    \end{flushleft}
  

==> examples/cpojer-js-codemod-jest-arrow-5.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^describe("describe", function () {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  it("should be happy", () => {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    console.log("actually forwards body");^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  });^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  it("should leave arrow functions", () => {});^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  describe^\strut\UseVerb{Verb}\SaveVerb{Verb}^("nested describe", () => {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    xit("disabled still counts", () => {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    xdescribe("disabled describe", () => {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  })^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^});^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^function containsit() {}^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^containsit(function () {});^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{\{}\hspace{2mm}\keys{\}}\hspace{2mm}\keys{c}\hspace{2mm}\keys{\arrowkeyup}\hspace{2mm}\keys{i}\\
Type \SaveVerb{Verb}^()=>{},^\adjustbox{bgcolor={HTML}{F2F2F2}}{\strut\UseVerb{Verb}}\\
\keys{\esc}\hspace{2mm}\keys{\{}\hspace{2mm}\keys{\}}\hspace{2mm}\keys{p}\hspace{2mm}\keys{\shift+\arrowkeyright}\hspace{2mm}\keys{\SPACE}\hspace{2mm}\keys{d}
    \end{flushleft}
  

==> examples/cpojer-js-codemod-jest-arrow-6.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^describe("describe", function () {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  it("should be happy", () => {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    console.log("actually forwards body");^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  });^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  it("should leave arrow functions", () => {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  describe("nested describe", () => {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    xit("disabled still counts", () => {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    xdescribe("disabled describe", () => {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  });^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^function containsit() {}^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^containsit(function () {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{)}\hspace{2mm}\keys{)}\hspace{2mm}\keys{)}\hspace{2mm}\keys{\arrowkeyup}\hspace{2mm}\keys{\arrowkeyup}\hspace{2mm}\keys{\shift+s}\hspace{2mm}\keys{f}
    \end{flushleft}
  

==> examples/cpojer-js-codemod-jest-arrow-7.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^describe("describe", function () {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  it("should be happy", () => {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    console.log("actually forwards body");^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  });^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  it("should leave arrow functions", () => {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  describe("nested describe", () => {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    xit("disabled still counts", () => {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    xdescribe("disabled describe", () => {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  });^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^})^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^function containsit() {}^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^containsit(function () {});^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      Use structural search UI (not shown) to find calls with callee names matching a regular expression and having a function expression as the second argument\\
\keys{\shift+s}\hspace{2mm}\keys{\arrowkeydown}
    \end{flushleft}
  

==> examples/cpojer-js-codemod-jest-arrow-8.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^describe^\strut\UseVerb{Verb}\SaveVerb{Verb}^("describe", () => {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  it("should be happy", () => {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    console.log("actually forwards body");^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  });^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  it("should leave arrow functions", () => {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  describe("nested describe", () => {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    xit("disabled still counts", () => {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    xdescribe("disabled describe", () => {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  });^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^})^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^function containsit() {}^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^containsit(function () {});^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{\{}\hspace{2mm}\keys{\}}\hspace{2mm}\keys{c}\hspace{2mm}\keys{\arrowkeyup}\hspace{2mm}\keys{i}\\
Type \SaveVerb{Verb}^()=>{},^\adjustbox{bgcolor={HTML}{F2F2F2}}{\strut\UseVerb{Verb}}\\
\keys{\esc}\hspace{2mm}\keys{\{}\hspace{2mm}\keys{\}}\hspace{2mm}\keys{p}\hspace{2mm}\keys{\shift+\arrowkeyright}\hspace{2mm}\keys{\SPACE}\hspace{2mm}\keys{d}
    \end{flushleft}
  

==> examples/cpojer-js-codemod-jest-arrow-9.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^describe("describe", () => {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  it("should be happy", () => {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    console.log("actually forwards body");^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  });^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  it("should leave existing arrow functions alone", () => {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  describe("nested describe", () => {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    xit("disabled one still count", () => {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    xdescribe("disabled describe as well", () => {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  });^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^})^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^function containsit() {}^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^containsit(function () {});^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{\}}\hspace{2mm}\keys{\}}\hspace{2mm}\keys{\}}\hspace{2mm}\keys{)}\hspace{2mm}\keys{\arrowkeyup}\hspace{2mm}\keys{\shift+s}\hspace{2mm}\keys{f}
    \end{flushleft}
  

==> examples/cpojer-js-codemod-jest-arrow-fail-0.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^describe("describe", function () {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  it("should be happy", function () {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    console.log("actually forwards body");^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  });^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  it("should leave arrow functions", () => {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  describe("nested describe", function () {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    xit("disabled still counts", function () {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    xdescribe("disabled describe", function () {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  });^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^function containsit() {}^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^containsit(function () {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      
    \end{flushleft}
  

==> examples/cpojer-js-codemod-jest-arrow-fail-1.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^describe("describe", function () {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  it("should be happy", function () {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    console.log("actually forwards body");^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  });^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  it("should leave arrow functions", () => {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  describe("nested describe", function () {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    xit("disabled still counts", function () {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    xdescribe("disabled describe", function () {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  });^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^})^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^function containsit() {}^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^containsit(function () {});^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      Use structural search UI (not shown) to find calls with callee names matching a regular expression and having a function expression as the second argument
    \end{flushleft}
  

==> examples/cpojer-js-codemod-jest-arrow-fail-2.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^describe("describe", function () ^\strut\UseVerb{Verb}\SaveVerb{Verb}^{^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  it("should be happy", function () {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    console.log("actually forwards body");^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  });^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  it("should leave arrow functions", () => {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  describe("nested describe", function () {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    xit("disabled still counts", function () {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    xdescribe("disabled describe", function () {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  });^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^}^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^function containsit() {}^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^containsit(function () {});^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{\{}\hspace{2mm}\keys{\}}\hspace{2mm}\keys{c}
    \end{flushleft}
  

==> examples/cpojer-js-codemod-jest-arrow-fail-3.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^describe(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  "describe",^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  () => ^\strut\UseVerb{Verb}\SaveVerb{Verb}^{^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    it("should be happy", function () {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^      console.log("actually forwards body");^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    });^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    it("should leave arrow functions", () => {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    describe("nested describe", function () {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^      xit("disabled still counts", function () {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^      xdescribe("disabled describe", function () {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    });^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  }^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  function () {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    it(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^      "should be happy",^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^      () => ^\strut\UseVerb{Verb}\SaveVerb{Verb}^{^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^        console.log("actually forwards body");^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^      }^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^      function () {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^        console.log("actually forwards body");^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^      },^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    );^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    it("should leave arrow functions", () => {});^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    describe(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^      "nested describe",^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^      () => ^\strut\UseVerb{Verb}\SaveVerb{Verb}^{^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^        xit("disabled still counts", function () {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^        xdescribe("disabled describe", function () {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^      }^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^      function () {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^        xit(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^          "disabled still counts",^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^          () => ^\strut\UseVerb{Verb}\SaveVerb{Verb}^{}^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^          function () {},^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^        );^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^        xdescribe(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^          "disabled describe",^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^          () => ^\strut\UseVerb{Verb}\SaveVerb{Verb}^{}^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^          function () {},^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^        );^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^      },^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    );^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  },^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^function containsit() {}^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^containsit(function () {});^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{\arrowkeyup}\hspace{2mm}\keys{i}\\
Type \SaveVerb{Verb}^()=>{},^\adjustbox{bgcolor={HTML}{F2F2F2}}{\strut\UseVerb{Verb}}\\
\keys{\esc}\hspace{2mm}\keys{\{}\hspace{2mm}\keys{\}}\hspace{2mm}\keys{p}
    \end{flushleft}
  

==> examples/cpojer-js-codemod-jest-arrow-fail-4.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^describe^\strut\UseVerb{Verb}\SaveVerb{Verb}^("describe", () => {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  it("should be happy", function () {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    console.log("actually forwards body");^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  });^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  it("should leave arrow functions", () => {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  describe("nested describe", function () {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    xit("disabled still counts", function () {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    xdescribe("disabled describe", function () {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  });^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^})^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^function containsit() {}^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^containsit(function () {});^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{\shift+\arrowkeyright}\hspace{2mm}\keys{\SPACE}\hspace{2mm}\keys{d}
    \end{flushleft}
  

==> examples/cpojer-js-codemod-jest-arrow-fail.tex <==

\FloatBarrier
\subsection{cpojer-js-codemod-jest-arrow-fail}
\label{example:cpojer-js-codemod-jest-arrow-fail}
\setcounter{figure}{0}

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-jest-arrow-fail-0.tex}
        \normalsize
        \captionof{figure}{Initial state}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-jest-arrow-fail-1.tex}
        \normalsize
        \captionof{figure}{Search for ``it'' and ``describe'' calls}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-jest-arrow-fail-2.tex}
        \normalsize
        \captionof{figure}{Copy function body}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-jest-arrow-fail-3.tex}
        \normalsize
        \captionof{figure}{Create arrow function and paste body. This is the problematic step. Changes from inner cursors are lost, because they were made after the function body was copied.}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-jest-arrow-fail-4.tex}
        \normalsize
        \captionof{figure}{Delete function expression}
        
      \end{examplestep}
    
\FloatBarrier
  

==> examples/cpojer-js-codemod-jest-arrow-flat-0.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^it("should be happy", function () {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  console.log("actually forwards body");^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^it("another one", function () {});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      
    \end{flushleft}
  

==> examples/cpojer-js-codemod-jest-arrow-flat-1.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^it("should be happy", ^\strut\UseVerb{Verb}\SaveVerb{Verb}^function () {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  console.log("actually forwards body");^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^}^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^it("another one", ^\strut\UseVerb{Verb}\SaveVerb{Verb}^function () {}^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^);^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      Use structural search UI (not shown) to search for function expressions (with any content)
    \end{flushleft}
  

==> examples/cpojer-js-codemod-jest-arrow-flat-2.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^it("should be happy", function () ^\strut\UseVerb{Verb}\SaveVerb{Verb}^{^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  console.log("actually forwards body");^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^}^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^it("another one", function () ^\strut\UseVerb{Verb}\SaveVerb{Verb}^{}^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^);^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{\{}\hspace{2mm}\keys{\}}\hspace{2mm}\keys{c}
    \end{flushleft}
  

==> examples/cpojer-js-codemod-jest-arrow-flat-3.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^it(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  "should be happy",^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  () => ^\strut\UseVerb{Verb}\SaveVerb{Verb}^{^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    console.log("actually forwards body");^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  }^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  function () {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    console.log("actually forwards body");^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  },^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^it(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  "another one",^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  () => ^\strut\UseVerb{Verb}\SaveVerb{Verb}^{}^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  function () {},^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^);^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{\arrowkeyup}\hspace{2mm}\keys{i}\\
Type \SaveVerb{Verb}^()=>{},^\adjustbox{bgcolor={HTML}{F2F2F2}}{\strut\UseVerb{Verb}}\\
\keys{\esc}\hspace{2mm}\keys{\{}\hspace{2mm}\keys{\}}\hspace{2mm}\keys{p}
    \end{flushleft}
  

==> examples/cpojer-js-codemod-jest-arrow-flat-4.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^it^\strut\UseVerb{Verb}\SaveVerb{Verb}^("should be happy", () => {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  console.log("actually forwards body");^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^})^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^it^\strut\UseVerb{Verb}\SaveVerb{Verb}^("another one", () => {})^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{\shift+\arrowkeyright}\hspace{2mm}\keys{\SPACE}\hspace{2mm}\keys{d}
    \end{flushleft}
  

==> examples/cpojer-js-codemod-jest-arrow-flat.tex <==

\FloatBarrier
\subsection{cpojer-js-codemod-jest-arrow-flat}
\label{example:cpojer-js-codemod-jest-arrow-flat}
\setcounter{figure}{0}

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-jest-arrow-flat-0.tex}
        \normalsize
        \captionof{figure}{Initial state}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-jest-arrow-flat-1.tex}
        \normalsize
        \captionof{figure}{Search for function expressions}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-jest-arrow-flat-2.tex}
        \normalsize
        \captionof{figure}{Copy function body}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-jest-arrow-flat-3.tex}
        \normalsize
        \captionof{figure}{Create arrow function and paste body}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-jest-arrow-flat-4.tex}
        \normalsize
        \captionof{figure}{Delete function expression}
        
      \end{examplestep}
    
\FloatBarrier
  

==> examples/cpojer-js-codemod-jest-arrow.tex <==

\FloatBarrier
\subsection{cpojer-js-codemod-jest-arrow}
\label{example:cpojer-js-codemod-jest-arrow}
\setcounter{figure}{0}

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-jest-arrow-0.tex}
        \normalsize
        \captionof{figure}{Initial state}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-jest-arrow-1.tex}
        \normalsize
        \captionof{figure}{Pass 1: Search for ``it`` and ``describe'' calls. Delete all cursors except innermost.}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-jest-arrow-2.tex}
        \normalsize
        \captionof{figure}{Pass 1: Copy function body. Create arrow function. Paste body. Delete function expression.}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-jest-arrow-3.tex}
        \normalsize
        \captionof{figure}{Select whole document and remove duplicate cursors.}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-jest-arrow-4.tex}
        \normalsize
        \captionof{figure}{Pass 2: Search for ``it`` and ``describe'' calls. Delete all cursors except innermost.}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-jest-arrow-5.tex}
        \normalsize
        \captionof{figure}{Pass 2: Copy function body. Create arrow function. Paste body. Delete function expression.}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-jest-arrow-6.tex}
        \normalsize
        \captionof{figure}{Select whole document and remove duplicate cursors.}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-jest-arrow-7.tex}
        \normalsize
        \captionof{figure}{Pass 3: Search for ``it`` and ``describe'' calls. Delete all cursors except innermost.}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-jest-arrow-8.tex}
        \normalsize
        \captionof{figure}{Pass 3: Copy function body. Create arrow function. Paste body. Delete function expression.}
        
      \end{examplestep}
    
\FloatBarrier
  

==> examples/cpojer-js-codemod-rm-object-assign-basic-0.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^let x = Object.assign({}, { a: 1 }, { b: 2 });^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^Object.assign({}, a);^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^Object.assign({ a: 1 }, b, { c: 3 });^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^Object.assign(a, b);^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^Object.assign({}, ...b);^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^Object.assign(^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    a: 1,^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  },^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  { b: 2 },^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  c,^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  d,^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^);^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      
    \end{flushleft}
  

==> examples/cpojer-js-codemod-rm-object-assign-basic-1.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^let x = Object.assign(^\strut\UseVerb{Verb}\SaveVerb{Verb}^{}, { a: 1 }, { b: 2 }^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign(^\strut\UseVerb{Verb}\SaveVerb{Verb}^{}, a^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign(^\strut\UseVerb{Verb}\SaveVerb{Verb}^{ a: 1 }, b, { c: 3 }^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign(^\strut\UseVerb{Verb}\SaveVerb{Verb}^a, b^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign(^\strut\UseVerb{Verb}\SaveVerb{Verb}^{}, ...b^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ^\strut\UseVerb{Verb}\SaveVerb{Verb}^{^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    a: 1,^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  },^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  { b: 2 },^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  c,^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  d^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^);^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{s}\hspace{2mm}\keys{(}\hspace{2mm}\keys{y}\hspace{2mm}\keys{s}
    \end{flushleft}
  

==> examples/cpojer-js-codemod-rm-object-assign-basic-2.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^let x = Object.assign(^\strut\UseVerb{Verb}\SaveVerb{Verb}^{}^\adjustbox{bgcolor={HTML}{C0EBB5}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, { a: 1 }, { b: 2 });^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign(^\strut\UseVerb{Verb}\SaveVerb{Verb}^{}^\adjustbox{bgcolor={HTML}{C0EBB5}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, a);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign(^\strut\UseVerb{Verb}\SaveVerb{Verb}^{ a: 1 }^\adjustbox{bgcolor={HTML}{C0EBB5}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, b, { c: 3 });^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign(^\strut\UseVerb{Verb}\SaveVerb{Verb}^a^\adjustbox{bgcolor={HTML}{FAB2B2}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, b);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign(^\strut\UseVerb{Verb}\SaveVerb{Verb}^{}^\adjustbox{bgcolor={HTML}{C0EBB5}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, ...b);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ^\strut\UseVerb{Verb}\SaveVerb{Verb}^{^\adjustbox{bgcolor={HTML}{C0EBB5}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    a: 1,^\adjustbox{bgcolor={HTML}{C0EBB5}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  }^\adjustbox{bgcolor={HTML}{C0EBB5}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  { b: 2 },^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  c,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  d,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^);^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{\Alt+\arrowkeyleft}\\
Use structural search UI (not shown) to check whether the selected node is an object literal\\
\keys{\shift+y}
    \end{flushleft}
  

==> examples/cpojer-js-codemod-rm-object-assign-basic-3.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^let x = Object.assign({}, ^\strut\UseVerb{Verb}\SaveVerb{Verb}^{ a: 1 }^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, { b: 2 }^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign({}, ^\strut\UseVerb{Verb}\SaveVerb{Verb}^a^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign({ a: 1 }, ^\strut\UseVerb{Verb}\SaveVerb{Verb}^b^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, { c: 3 }^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign(a, b);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign({}, ^\strut\UseVerb{Verb}\SaveVerb{Verb}^...b^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    a: 1,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  },^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ^\strut\UseVerb{Verb}\SaveVerb{Verb}^{ b: 2 }^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  c,^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  d^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^);^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{s}\hspace{2mm}\keys{\arrowkeyup}\hspace{2mm}\keys{\ctrl+\shift+\arrowkeyright}
    \end{flushleft}
  

==> examples/cpojer-js-codemod-rm-object-assign-basic-4.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^let x = Object.assign({}, ^\strut\UseVerb{Verb}\SaveVerb{Verb}^{ a: 1 }^\adjustbox{bgcolor={HTML}{FAB2B2}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, { b: 2 }^\adjustbox{bgcolor={HTML}{FAB2B2}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign({}, ^\strut\UseVerb{Verb}\SaveVerb{Verb}^a^\adjustbox{bgcolor={HTML}{FAB2B2}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign({ a: 1 }, ^\strut\UseVerb{Verb}\SaveVerb{Verb}^b^\adjustbox{bgcolor={HTML}{FAB2B2}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, { c: 3 }^\adjustbox{bgcolor={HTML}{FAB2B2}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign(a, b);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign({}, ^\strut\UseVerb{Verb}\SaveVerb{Verb}^...b^\adjustbox{bgcolor={HTML}{C0EBB5}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    a: 1,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  },^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ^\strut\UseVerb{Verb}\SaveVerb{Verb}^{ b: 2 }^\adjustbox{bgcolor={HTML}{FAB2B2}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\adjustbox{bgcolor={HTML}{FAB2B2}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  c,^\adjustbox{bgcolor={HTML}{FAB2B2}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  d^\adjustbox{bgcolor={HTML}{FAB2B2}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^);^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      Use structural search UI (not shown) to search for spread elements\\
\keys{\shift+y}
    \end{flushleft}
  

==> examples/cpojer-js-codemod-rm-object-assign-basic-5.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^let x = Object.assign(^\strut\UseVerb{Verb}\SaveVerb{Verb}^{}^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, ^\strut\UseVerb{Verb}\SaveVerb{Verb}^{ a: 1 }^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, ^\strut\UseVerb{Verb}\SaveVerb{Verb}^{ b: 2 }^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, {});^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign(^\strut\UseVerb{Verb}\SaveVerb{Verb}^{}^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, ^\strut\UseVerb{Verb}\SaveVerb{Verb}^a^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, {});^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign(^\strut\UseVerb{Verb}\SaveVerb{Verb}^{ a: 1 }^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, ^\strut\UseVerb{Verb}\SaveVerb{Verb}^b^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, ^\strut\UseVerb{Verb}\SaveVerb{Verb}^{ c: 3 }^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, {});^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign(a, b);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign({}, ...b);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign(^\strut\UseVerb{Verb}\SaveVerb{Verb}^{ a: 1 }^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, ^\strut\UseVerb{Verb}\SaveVerb{Verb}^{ b: 2 }^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, ^\strut\UseVerb{Verb}\SaveVerb{Verb}^c^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, ^\strut\UseVerb{Verb}\SaveVerb{Verb}^d^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, {});^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{f}\hspace{2mm}\keys{\arrowkeyup}\hspace{2mm}\keys{a}\\
Type \SaveVerb{Verb}^,{}^\adjustbox{bgcolor={HTML}{F2F2F2}}{\strut\UseVerb{Verb}}\\
\keys{\esc}\hspace{2mm}\keys{\arrowkeyup}\hspace{2mm}\keys{\ctrl+\shift+\arrowkeyleft}\hspace{2mm}\keys{s}
    \end{flushleft}
  

==> examples/cpojer-js-codemod-rm-object-assign-basic-6.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^let x = Object.assign(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  {},^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  { a: 1 },^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  { b: 2 },^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  { ...(^\strut\UseVerb{Verb}\SaveVerb{Verb}^{}^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^), ...(^\strut\UseVerb{Verb}\SaveVerb{Verb}^{ a: 1 }^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^), ...(^\strut\UseVerb{Verb}\SaveVerb{Verb}^{ b: 2 }^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^) },^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign({}, a, { ...(^\strut\UseVerb{Verb}\SaveVerb{Verb}^{}^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^), ...(^\strut\UseVerb{Verb}\SaveVerb{Verb}^a^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^) });^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  { a: 1 },^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  b,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  { c: 3 },^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  { ...(^\strut\UseVerb{Verb}\SaveVerb{Verb}^{ a: 1 }^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^), ...(^\strut\UseVerb{Verb}\SaveVerb{Verb}^b^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^), ...(^\strut\UseVerb{Verb}\SaveVerb{Verb}^{ c: 3 }^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^) },^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign(a, b);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign({}, ...b);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign({ a: 1 }, { b: 2 }, c, d, {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ...(^\strut\UseVerb{Verb}\SaveVerb{Verb}^{ a: 1 }^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^),^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ...(^\strut\UseVerb{Verb}\SaveVerb{Verb}^{ b: 2 }^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^),^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ...(^\strut\UseVerb{Verb}\SaveVerb{Verb}^c^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^),^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ...(^\strut\UseVerb{Verb}\SaveVerb{Verb}^d^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^),^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^});^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{c}\hspace{2mm}\keys{)}\hspace{2mm}\keys{\Alt+\arrowkeyright}\hspace{2mm}\keys{\{}\hspace{2mm}\keys{a}\\
Type \SaveVerb{Verb}^...(x),^\adjustbox{bgcolor={HTML}{F2F2F2}}{\strut\UseVerb{Verb}}\\
\keys{\esc}\hspace{2mm}\keys{(}\hspace{2mm}\keys{p}
    \end{flushleft}
  

==> examples/cpojer-js-codemod-rm-object-assign-basic-7.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^let x =^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ^\strut\UseVerb{Verb}\SaveVerb{Verb}^(x) &&^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  Object.assign(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    {},^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    { a: 1 },^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    { b: 2 },^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    { ...({}), ...({ a: 1 }), ...({ b: 2 }) },^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  );^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^(x) &&^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^ Object.assign({}, a, { ...({}), ...(a) });^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^(x) &&^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  Object.assign(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    { a: 1 },^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    b,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    { c: 3 },^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    { ...({ a: 1 }), ...(b), ...({ c: 3 }) },^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  );^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign(a, b);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign({}, ...b);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^(x) &&^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  Object.assign({ a: 1 }, { b: 2 }, c, d, {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    ...({ a: 1 }),^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    ...({ b: 2 }),^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    ...(c),^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    ...(d),^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  });^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{\shift+s}\hspace{2mm}\keys{\arrowkeyleft}\hspace{2mm}\keys{\}}\hspace{2mm}\keys{c}\hspace{2mm}\keys{)}\hspace{2mm}\keys{\arrowkeyup}\hspace{2mm}\keys{i}\\
Type \SaveVerb{Verb}^(x) &&^\adjustbox{bgcolor={HTML}{F2F2F2}}{\strut\UseVerb{Verb}}\\
\keys{\esc}
    \end{flushleft}
  

==> examples/cpojer-js-codemod-rm-object-assign-basic-8.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^let x = ({ ...^\strut\UseVerb{Verb}\SaveVerb{Verb}^({})^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, ...^\strut\UseVerb{Verb}\SaveVerb{Verb}^({ a: 1 })^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, ...^\strut\UseVerb{Verb}\SaveVerb{Verb}^({ b: 2 })^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^ });^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^({ ...^\strut\UseVerb{Verb}\SaveVerb{Verb}^({})^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, ...^\strut\UseVerb{Verb}\SaveVerb{Verb}^(a)^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^ });^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^({ ...^\strut\UseVerb{Verb}\SaveVerb{Verb}^({ a: 1 })^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, ...^\strut\UseVerb{Verb}\SaveVerb{Verb}^(b)^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, ...^\strut\UseVerb{Verb}\SaveVerb{Verb}^({ c: 3 })^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^ });^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign(a, b);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^Object.assign({}, ...b);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^({ ...^\strut\UseVerb{Verb}\SaveVerb{Verb}^({ a: 1 })^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, ...^\strut\UseVerb{Verb}\SaveVerb{Verb}^({ b: 2 })^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, ...^\strut\UseVerb{Verb}\SaveVerb{Verb}^(c)^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, ...^\strut\UseVerb{Verb}\SaveVerb{Verb}^(d)^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^ });^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{(}\hspace{2mm}\keys{p}\hspace{2mm}\keys{)}\hspace{2mm}\keys{\arrowkeyup}\hspace{2mm}\keys{\ctrl+\shift+\arrowkeyright}\hspace{2mm}\keys{d}\hspace{2mm}\keys{\{}\hspace{2mm}\keys{s}\hspace{2mm}\keys{\Alt+\arrowkeyright}
    \end{flushleft}
  

==> examples/cpojer-js-codemod-rm-object-assign-basic.tex <==

\FloatBarrier
\subsection{cpojer-js-codemod-rm-object-assign-basic}
\label{example:cpojer-js-codemod-rm-object-assign-basic}
\setcounter{figure}{0}

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-rm-object-assign-basic-0.tex}
        \normalsize
        \captionof{figure}{Initial state}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-rm-object-assign-basic-1.tex}
        \normalsize
        \captionof{figure}{Split cursors (one per call) and select its arguments. Switch to multi-cursor strict mode.}
        \label{step:cpojer-js-codemod-rm-object-assign-basic:get-object-assign}
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-rm-object-assign-basic-2.tex}
        \normalsize
        \captionof{figure}{Check whether first argument is an object and show successful/failed cursors}
        \label{step:cpojer-js-codemod-rm-object-assign-basic:check-object-literal}
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-rm-object-assign-basic-3.tex}
        \normalsize
        \captionof{figure}{Keep successful cursors. Select all arguments except first.}
        \label{step:cpojer-js-codemod-rm-object-assign-basic:keep-object-literal}
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-rm-object-assign-basic-4.tex}
        \normalsize
        \captionof{figure}{Search for spread elements and show successful/failed cursors}
        \label{step:cpojer-js-codemod-rm-object-assign-basic:check-spread}
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-rm-object-assign-basic-5.tex}
        \normalsize
        \captionof{figure}{Keep failed cursors. Append object literal to argument list. Select other arguments and split cursor (one for each old argument).}
        \label{step:cpojer-js-codemod-rm-object-assign-basic:keep-no-spread}
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-rm-object-assign-basic-6.tex}
        \normalsize
        \captionof{figure}{Copy argument. Insert placeholder spread element into object. Paste argument.}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-rm-object-assign-basic-7.tex}
        \normalsize
        \captionof{figure}{Remove all cursors except first. Copy new object literal. Insert placeholder where it will later be pasted.}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-rm-object-assign-basic-8.tex}
        \normalsize
        \captionof{figure}{Paste object literal and delete ``Object.assign'' call.}
        
      \end{examplestep}
    
\FloatBarrier
  

==> examples/cpojer-js-codemod-unchain-variables-0.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^var foo = true,^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  bar = false;^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^const baz = 1,^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  fiz = "2";^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^let buzz = 3.3,^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  biz = {};^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^var hello,^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  ohai = function ohai() {},^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  hi;^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^var Neil, deGrasse, Tyson;^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^for (var i = 0, j = 10; i < j; i++, j--) {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  console.log(i, j);^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^}^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      
    \end{flushleft}
  

==> examples/cpojer-js-codemod-unchain-variables-1.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^var foo = true,^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  bar = false^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^const baz = 1,^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  fiz = "2"^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^let buzz = 3.3,^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  biz = {}^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var hello,^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  ohai = function ohai() {},^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  hi^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var Neil, deGrasse, Tyson^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^for (var i = 0, j = 10; i < j; i++, j--) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  console.log(i, j);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^}^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{\ctrl+\shift+\arrowkeyleft}\hspace{2mm}\keys{s}
    \end{flushleft}
  

==> examples/cpojer-js-codemod-unchain-variables-2.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^var ^\strut\UseVerb{Verb}\SaveVerb{Verb}^foo = true^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ^\strut\UseVerb{Verb}\SaveVerb{Verb}^bar = false^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^const ^\strut\UseVerb{Verb}\SaveVerb{Verb}^baz = 1^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ^\strut\UseVerb{Verb}\SaveVerb{Verb}^fiz = "2"^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^let ^\strut\UseVerb{Verb}\SaveVerb{Verb}^buzz = 3.3^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ^\strut\UseVerb{Verb}\SaveVerb{Verb}^biz = {}^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var ^\strut\UseVerb{Verb}\SaveVerb{Verb}^hello^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ^\strut\UseVerb{Verb}\SaveVerb{Verb}^ohai = function ohai() {}^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ^\strut\UseVerb{Verb}\SaveVerb{Verb}^hi^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var ^\strut\UseVerb{Verb}\SaveVerb{Verb}^Neil^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, ^\strut\UseVerb{Verb}\SaveVerb{Verb}^deGrasse^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, ^\strut\UseVerb{Verb}\SaveVerb{Verb}^Tyson^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^for (var i = 0, j = 10; i < j; i++, j--) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  console.log(i, j);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^}^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{\ctrl+\shift+\arrowkeyright}\hspace{2mm}\keys{s}\hspace{2mm}\keys{m}\hspace{2mm}\keys{a}\hspace{2mm}\keys{c}
    \end{flushleft}
  

==> examples/cpojer-js-codemod-unchain-variables-3.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^var foo = true,^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  bar = false^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^const baz = 1,^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  fiz = "2"^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^let buzz = 3.3,^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  biz = {}^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var hello,^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  ohai = function ohai() {},^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  hi^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var Neil, deGrasse, Tyson^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^for (var i = 0, j = 10; i < j; i++, j--) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  console.log(i, j);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^}^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{\arrowkeyup}
    \end{flushleft}
  

==> examples/cpojer-js-codemod-unchain-variables-4.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^var x^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var x^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var foo = true,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  bar = false;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var x^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var x^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^const baz = 1,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  fiz = "2";^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var x^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var x^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^let buzz = 3.3,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  biz = {};^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var x^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var x^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var x^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var hello,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ohai = function ohai() {},^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  hi;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var x^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var x^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var x^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var Neil, deGrasse, Tyson;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^for (var i = 0, j = 10; i < j; i++, j--) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  console.log(i, j);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^}^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{i}\\
Type \SaveVerb{Verb}^var x;^\adjustbox{bgcolor={HTML}{F2F2F2}}{\strut\UseVerb{Verb}}\\
\keys{\esc}
    \end{flushleft}
  

==> examples/cpojer-js-codemod-unchain-variables-5.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^var ^\strut\UseVerb{Verb}\SaveVerb{Verb}^foo = true^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var ^\strut\UseVerb{Verb}\SaveVerb{Verb}^bar = false^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var foo = true,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  bar = false;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var ^\strut\UseVerb{Verb}\SaveVerb{Verb}^baz = 1^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var ^\strut\UseVerb{Verb}\SaveVerb{Verb}^fiz = "2"^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^const baz = 1,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  fiz = "2";^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var ^\strut\UseVerb{Verb}\SaveVerb{Verb}^buzz = 3.3^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var ^\strut\UseVerb{Verb}\SaveVerb{Verb}^biz = {}^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^let buzz = 3.3,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  biz = {};^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var ^\strut\UseVerb{Verb}\SaveVerb{Verb}^hello^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var ^\strut\UseVerb{Verb}\SaveVerb{Verb}^ohai = function ohai() {}^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var ^\strut\UseVerb{Verb}\SaveVerb{Verb}^hi^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var hello,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ohai = function ohai() {},^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  hi;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var ^\strut\UseVerb{Verb}\SaveVerb{Verb}^Neil^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var ^\strut\UseVerb{Verb}\SaveVerb{Verb}^deGrasse^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var ^\strut\UseVerb{Verb}\SaveVerb{Verb}^Tyson^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var Neil, deGrasse, Tyson;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^for (var i = 0, j = 10; i < j; i++, j--) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  console.log(i, j);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^}^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{\Alt+\arrowkeyright}\hspace{2mm}\keys{p}\hspace{2mm}\keys{m}\hspace{2mm}\keys{b}
    \end{flushleft}
  

==> examples/cpojer-js-codemod-unchain-variables-6.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^var^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^ foo = true;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^ bar = false;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var foo = true,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  bar = false;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^const^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^ baz = 1;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^const^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^ fiz = "2";^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^const baz = 1,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  fiz = "2";^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^let^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^ buzz = 3.3;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^let^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^ biz = {};^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^let buzz = 3.3,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  biz = {};^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^ hello;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^ ohai = function ohai() {};^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^ hi;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var hello,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ohai = function ohai() {},^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  hi;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^ Neil;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^ deGrasse;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^ Tyson;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^var Neil, deGrasse, Tyson;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^for (var i = 0, j = 10; i < j; i++, j--) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  console.log(i, j);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^}^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{\shift+m}\hspace{2mm}\keys{a}\hspace{2mm}\keys{\arrowkeyup}\hspace{2mm}\keys{\Alt+\arrowkeyleft}\hspace{2mm}\keys{c}\hspace{2mm}\keys{\shift+m}\hspace{2mm}\keys{b}\hspace{2mm}\keys{\arrowkeyleft}\hspace{2mm}\keys{p}
    \end{flushleft}
  

==> examples/cpojer-js-codemod-unchain-variables-7.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^var foo = true;^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^var bar = false;^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^const baz = 1;^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^const fiz = "2";^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^let buzz = 3.3;^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^let biz = {};^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^var hello;^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^var ohai = function ohai() {};^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^var hi;^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^var Neil;^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^var deGrasse;^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^var Tyson;^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^for (var i = 0, j = 10; i < j; i++, j--) {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  console.log(i, j);^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^}^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{\shift+s}\hspace{2mm}\keys{\arrowkeyleft}\hspace{2mm}\keys{\shift+m}\hspace{2mm}\keys{a}\hspace{2mm}\keys{\arrowkeyup}\hspace{2mm}\keys{d}
    \end{flushleft}
  

==> examples/cpojer-js-codemod-unchain-variables.tex <==

\FloatBarrier
\subsection{cpojer-js-codemod-unchain-variables}
\label{example:cpojer-js-codemod-unchain-variables}
\setcounter{figure}{0}

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-unchain-variables-0.tex}
        \normalsize
        \captionof{figure}{Initial state}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-unchain-variables-1.tex}
        \normalsize
        \captionof{figure}{Deselect for loop. Split cursor (one per statement).}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-unchain-variables-2.tex}
        \normalsize
        \captionof{figure}{Deselect keyword. Split cursor (one per declaration). Mark and copy declaration.}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-unchain-variables-3.tex}
        \normalsize
        \captionof{figure}{Move up to statement (cursors overlap)}
        \label{step:cpojer-js-codemod-unchain-variables:statement-overlap}
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-unchain-variables-4.tex}
        \normalsize
        \captionof{figure}{Insert new statements (multiple copies inserted due to overlapping cursors)}
        \label{step:cpojer-js-codemod-unchain-variables:insert}
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-unchain-variables-5.tex}
        \normalsize
        \captionof{figure}{Paste declaration into new statement and mark the paste location}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-unchain-variables-6.tex}
        \normalsize
        \captionof{figure}{Go to old keyword, copy it, and jump back, and paste it.}
        \label{step:cpojer-js-codemod-unchain-variables:keyword-overlap}
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/cpojer-js-codemod-unchain-variables-7.tex}
        \normalsize
        \captionof{figure}{Delete all cursors except the first (per old statement). Delete the old statement.}
        
      \end{examplestep}
    
\FloatBarrier
  

==> examples/index.tex <==
\input{examples/multi-cursor-reduce-across}\clearpage
\input{examples/multi-cursor-marks}\clearpage
\input{examples/cpojer-js-codemod-unchain-variables}\clearpage
\input{examples/cpojer-js-codemod-jest-arrow-flat}\clearpage
\input{examples/cpojer-js-codemod-jest-arrow-fail}\clearpage
% \input{examples/cpojer-js-codemod-jest-arrow}\clearpage
\input{examples/cpojer-js-codemod-rm-object-assign-basic}\clearpage
% \input{examples/wrap-handlers}\clearpage

==> examples/multi-cursor-marks-0.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^export function f(^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  thing: string = "test",^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  count: number = 1,^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^) {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  return count === 1 ? thing : thing + "s";^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^}^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      
    \end{flushleft}
  

==> examples/multi-cursor-marks-1.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^export function f(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  thing: string = "test",^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  count: number = 1,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ^\strut\UseVerb{Verb}\SaveVerb{Verb}^if (debug) {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    console.log({});^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  }^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  return count === 1 ? thing : thing + "s";^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^}^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{\{}\hspace{2mm}\keys{i}\\
Type \SaveVerb{Verb}^if(debug){console.log({})}^\adjustbox{bgcolor={HTML}{F2F2F2}}{\strut\UseVerb{Verb}}\\
\keys{\esc}
    \end{flushleft}
  

==> examples/multi-cursor-marks-10.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^export function f(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  thing: string = "test",^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  count: number = 1,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  debug: boolean = false,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  if (debug) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    console.log({^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^      thing: { current: thing, default: ^\strut\UseVerb{Verb}\SaveVerb{Verb}^"test"^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^ },^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^      count: { current: count, default: ^\strut\UseVerb{Verb}\SaveVerb{Verb}^1^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^ },^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    });^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  }^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  return count === 1 ? thing : thing + "s";^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^}^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{\shift+m}\hspace{2mm}\keys{c}\hspace{2mm}\keys{p}
    \end{flushleft}
  

==> examples/multi-cursor-marks-2.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^export function f(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  thing: string = "test",^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  count: number = 1,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  if (debug) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    console.log(^\strut\UseVerb{Verb}\SaveVerb{Verb}^{}^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  }^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  return count === 1 ? thing : thing + "s";^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^}^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{\{}\hspace{2mm}\keys{\{}\hspace{2mm}\keys{\}}\hspace{2mm}\keys{m}\hspace{2mm}\keys{a}
    \end{flushleft}
  

==> examples/multi-cursor-marks-3.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^export function f(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  thing: string = "test",^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  count: number = 1,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ^\strut\UseVerb{Verb}\SaveVerb{Verb}^debug: boolean = false^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  if (debug) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    console.log({});^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  }^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  return count === 1 ? thing : thing + "s";^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^}^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{\}}\hspace{2mm}\keys{\}}\hspace{2mm}\keys{\shift+\arrowkeyleft}\hspace{2mm}\keys{\SPACE}\hspace{2mm}\keys{\arrowkeydown}\hspace{2mm}\keys{a}\\
Type \SaveVerb{Verb}^,debug:boolean=false^\adjustbox{bgcolor={HTML}{F2F2F2}}{\strut\UseVerb{Verb}}\\
\keys{\esc}
    \end{flushleft}
  

==> examples/multi-cursor-marks-4.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^export function f(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ^\strut\UseVerb{Verb}\SaveVerb{Verb}^thing: string = "test"^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ^\strut\UseVerb{Verb}\SaveVerb{Verb}^count: number = 1^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  debug: boolean = false,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  if (debug) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    console.log({});^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  }^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  return count === 1 ? thing : thing + "s";^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^}^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{\arrowkeyup}\hspace{2mm}\keys{\ctrl+\shift+\arrowkeyleft}\hspace{2mm}\keys{s}
    \end{flushleft}
  

==> examples/multi-cursor-marks-5.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^export function f(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ^\strut\UseVerb{Verb}\SaveVerb{Verb}^thing^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^: string = "test",^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ^\strut\UseVerb{Verb}\SaveVerb{Verb}^count^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^: number = 1,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  debug: boolean = false,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  if (debug) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    console.log({});^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  }^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  return count === 1 ? thing : thing + "s";^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^}^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{m}\hspace{2mm}\keys{b}\hspace{2mm}\keys{\Alt+\arrowkeyleft}\hspace{2mm}\keys{c}
    \end{flushleft}
  

==> examples/multi-cursor-marks-6.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^export function f(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  thing: string = "test",^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  count: number = 1,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  debug: boolean = false,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  if (debug) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    console.log({^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^      ^\strut\UseVerb{Verb}\SaveVerb{Verb}^x: { current: x, default: x }^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^      ^\strut\UseVerb{Verb}\SaveVerb{Verb}^x: { current: x, default: x }^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    });^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  }^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  return count === 1 ? thing : thing + "s";^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^}^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{\shift+m}\hspace{2mm}\keys{a}\hspace{2mm}\keys{\arrowkeydown}\hspace{2mm}\keys{a}\\
Type \SaveVerb{Verb}^x: {current: x, default: x},^\adjustbox{bgcolor={HTML}{F2F2F2}}{\strut\UseVerb{Verb}}\\
\keys{\esc}
    \end{flushleft}
  

==> examples/multi-cursor-marks-7.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^export function f(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  thing: string = "test",^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  count: number = 1,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  debug: boolean = false,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  if (debug) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    console.log({^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^      thing: { current: ^\strut\UseVerb{Verb}\SaveVerb{Verb}^thing^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, default: x },^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^      count: { current: ^\strut\UseVerb{Verb}\SaveVerb{Verb}^count^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, default: x },^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    });^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  }^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  return count === 1 ? thing : thing + "s";^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^}^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{\Alt+\arrowkeyleft}\hspace{2mm}\keys{p}\hspace{2mm}\keys{\arrowkeyright}\hspace{2mm}\keys{\arrowkeyright}\hspace{2mm}\keys{p}
    \end{flushleft}
  

==> examples/multi-cursor-marks-8.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^export function f(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  thing: string = "test",^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  count: number = 1,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  debug: boolean = false,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  if (debug) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    console.log({^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^      thing: { current: thing, default: ^\strut\UseVerb{Verb}\SaveVerb{Verb}^x^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^ },^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^      count: { current: count, default: ^\strut\UseVerb{Verb}\SaveVerb{Verb}^x^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^ },^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    });^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  }^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  return count === 1 ? thing : thing + "s";^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^}^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{\arrowkeyright}\hspace{2mm}\keys{\arrowkeyright}\hspace{2mm}\keys{m}\hspace{2mm}\keys{c}
    \end{flushleft}
  

==> examples/multi-cursor-marks-9.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^export function f(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  thing: string = ^\strut\UseVerb{Verb}\SaveVerb{Verb}^"test"^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  count: number = ^\strut\UseVerb{Verb}\SaveVerb{Verb}^1^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  debug: boolean = false,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  if (debug) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    console.log({^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^      thing: { current: thing, default: x },^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^      count: { current: count, default: x },^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    });^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  }^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  return count === 1 ? thing : thing + "s";^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^}^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{\shift+m}\hspace{2mm}\keys{b}\hspace{2mm}\keys{\Alt+\arrowkeyright}\hspace{2mm}\keys{c}
    \end{flushleft}
  

==> examples/multi-cursor-marks.tex <==

\FloatBarrier
\subsection{multi-cursor-marks}
\label{example:multi-cursor-marks}
\setcounter{figure}{0}

      \begin{examplestep}
        \small
        \input{examples/multi-cursor-marks-0.tex}
        \normalsize
        \captionof{figure}{Initial state}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/multi-cursor-marks-1.tex}
        \normalsize
        \captionof{figure}{Insert at start of function body}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/multi-cursor-marks-2.tex}
        \normalsize
        \captionof{figure}{Select and mark empty object literal}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/multi-cursor-marks-3.tex}
        \normalsize
        \captionof{figure}{Append function parameter}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/multi-cursor-marks-4.tex}
        \normalsize
        \captionof{figure}{Select parameters except debug and split cursor}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/multi-cursor-marks-5.tex}
        \normalsize
        \captionof{figure}{Mark parameter and copy parameter name}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/multi-cursor-marks-6.tex}
        \normalsize
        \captionof{figure}{Insert inside marked empty object literal}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/multi-cursor-marks-7.tex}
        \normalsize
        \captionof{figure}{Paste name over first two "x"s}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/multi-cursor-marks-8.tex}
        \normalsize
        \captionof{figure}{Move to last "x" and mark it}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/multi-cursor-marks-9.tex}
        \normalsize
        \captionof{figure}{Jump to marked parameter declaration and copy initializer}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/multi-cursor-marks-10.tex}
        \normalsize
        \captionof{figure}{Jump to last "x" and paste initializer}
        
      \end{examplestep}
    
\FloatBarrier
  

==> examples/multi-cursor-reduce-across-0.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^export function f(a, b, c) {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  return a * b * c;^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^}^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^export function g(a, b, c) {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  return a + b + c;^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^}^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      
    \end{flushleft}
  

==> examples/multi-cursor-reduce-across-1.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^export function f(a, b, c) {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  return a * b * c;^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^}^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^export function g(a, b, c) {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  return a + b + c;^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^}^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{s}
    \end{flushleft}
  

==> examples/multi-cursor-reduce-across-2.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^export function f(^\strut\UseVerb{Verb}\SaveVerb{Verb}^a^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, ^\strut\UseVerb{Verb}\SaveVerb{Verb}^b^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, ^\strut\UseVerb{Verb}\SaveVerb{Verb}^c^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  return a * b * c;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^}^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^export function g(^\strut\UseVerb{Verb}\SaveVerb{Verb}^a^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, ^\strut\UseVerb{Verb}\SaveVerb{Verb}^b^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^, ^\strut\UseVerb{Verb}\SaveVerb{Verb}^c^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  return a + b + c;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^}^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{(}\hspace{2mm}\keys{s}
    \end{flushleft}
  

==> examples/multi-cursor-reduce-across-3.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^export function f(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  a: ^\strut\UseVerb{Verb}\SaveVerb{Verb}^number^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  b: ^\strut\UseVerb{Verb}\SaveVerb{Verb}^number^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  c: ^\strut\UseVerb{Verb}\SaveVerb{Verb}^number^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  return a * b * c;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^}^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^export function g(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  a: ^\strut\UseVerb{Verb}\SaveVerb{Verb}^number^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  b: ^\strut\UseVerb{Verb}\SaveVerb{Verb}^number^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  c: ^\strut\UseVerb{Verb}\SaveVerb{Verb}^number^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  return a + b + c;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^}^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{a}\\
Type \SaveVerb{Verb}^:number^\adjustbox{bgcolor={HTML}{F2F2F2}}{\strut\UseVerb{Verb}}\\
\keys{\esc}
    \end{flushleft}
  

==> examples/multi-cursor-reduce-across-4.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^export function f(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  a: ^\strut\UseVerb{Verb}\SaveVerb{Verb}^number^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  b: number,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  c: number,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  return a * b * c;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^}^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^export function g(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  a: ^\strut\UseVerb{Verb}\SaveVerb{Verb}^number^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  b: number,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  c: number,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  return a + b + c;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^}^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{\shift+s}\hspace{2mm}\keys{\arrowkeyleft}
    \end{flushleft}
  

==> examples/multi-cursor-reduce-across-5.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^export function f(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  a: number,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  b: number,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  c: number,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^): ^\strut\UseVerb{Verb}\SaveVerb{Verb}^number^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^ {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  return a * b * c;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^}^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^export function g(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  a: number,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  b: number,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  c: number,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^): ^\strut\UseVerb{Verb}\SaveVerb{Verb}^number^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^ {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  return a + b + c;^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^}^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{)}\hspace{2mm}\keys{a}\\
Type \SaveVerb{Verb}^:number^\adjustbox{bgcolor={HTML}{F2F2F2}}{\strut\UseVerb{Verb}}\\
\keys{\esc}
    \end{flushleft}
  

==> examples/multi-cursor-reduce-across.tex <==

\FloatBarrier
\subsection{multi-cursor-reduce-across}
\label{example:multi-cursor-reduce-across}
\setcounter{figure}{0}

      \begin{examplestep}
        \small
        \input{examples/multi-cursor-reduce-across-0.tex}
        \normalsize
        \captionof{figure}{Initial state}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/multi-cursor-reduce-across-1.tex}
        \normalsize
        \captionof{figure}{Split cursor (one per function)}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/multi-cursor-reduce-across-2.tex}
        \normalsize
        \captionof{figure}{Go to parameters and split cursor (one per parameter)}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/multi-cursor-reduce-across-3.tex}
        \normalsize
        \captionof{figure}{Add type annotation to parameter}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/multi-cursor-reduce-across-4.tex}
        \normalsize
        \captionof{figure}{Remove all cursors except the first (per function)}
        \label{step:multi-cursor-reduce-across:reduce}
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/multi-cursor-reduce-across-5.tex}
        \normalsize
        \captionof{figure}{Add return type annotation}
        
      \end{examplestep}
    
\FloatBarrier
  

==> examples/wrap-handlers-0.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^export const handlers = {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  "ctrl-v": node.actions.setVariant^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    ? tryAction("setVariant", (n) => n.id, true)^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    : tryAction("setFromString"),^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  "ctrl-d": tryDeleteChild,^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  "ctrl-c": () => copyNode(node),^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  "ctrl-p": tryAction("replace", (n) => n.id),^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  "ctrl-f": editFlags,^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  "ctrl-4": () =>^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    setMarks({^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^      ...marks,^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^      TODO: idPathFromParentIndexEntry(^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^        parentIndexEntry,^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^      ),^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    }),^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^};^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^for (const [k, v] of handlers) {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  handlers[k] = warnOnError(v);^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^}^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      
    \end{flushleft}
  

==> examples/wrap-handlers-1.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^export const handlers = {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ^\strut\UseVerb{Verb}\SaveVerb{Verb}^"ctrl-v": node.actions.setVariant^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    ? tryAction("setVariant", (n) => n.id, true)^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    : tryAction("setFromString")^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ^\strut\UseVerb{Verb}\SaveVerb{Verb}^"ctrl-d": tryDeleteChild^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ^\strut\UseVerb{Verb}\SaveVerb{Verb}^"ctrl-c": () => copyNode(node)^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ^\strut\UseVerb{Verb}\SaveVerb{Verb}^"ctrl-p": tryAction("replace", (n) => n.id)^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ^\strut\UseVerb{Verb}\SaveVerb{Verb}^"ctrl-f": editFlags^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ^\strut\UseVerb{Verb}\SaveVerb{Verb}^"ctrl-4": () =>^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    setMarks({^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^      ...marks,^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^      TODO: idPathFromParentIndexEntry(^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^        parentIndexEntry,^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^      ),^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    })^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^};^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^for (const [k, v] of handlers) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  handlers[k] = warnOnError(v);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^}^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{\{}\hspace{2mm}\keys{s}
    \end{flushleft}
  

==> examples/wrap-handlers-2.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^export const handlers = {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ^\strut\UseVerb{Verb}\SaveVerb{Verb}^"ctrl-v": ^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^placeholder^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ^\strut\UseVerb{Verb}\SaveVerb{Verb}^"ctrl-d": ^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^placeholder^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ^\strut\UseVerb{Verb}\SaveVerb{Verb}^"ctrl-c": ^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^placeholder^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ^\strut\UseVerb{Verb}\SaveVerb{Verb}^"ctrl-p": ^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^placeholder^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ^\strut\UseVerb{Verb}\SaveVerb{Verb}^"ctrl-f": ^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^placeholder^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ^\strut\UseVerb{Verb}\SaveVerb{Verb}^"ctrl-4": ^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^placeholder^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^};^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^for (const [k, v] of handlers) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  handlers[k] = warnOnError(v);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^}^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{\Alt+\arrowkeyright}\hspace{2mm}\keys{c}\hspace{2mm}\keys{d}
    \end{flushleft}
  

==> examples/wrap-handlers-3.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^export const handlers = {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  "ctrl-v": warnOnError(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    ^\strut\UseVerb{Verb}\SaveVerb{Verb}^node.actions.setVariant^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^      ? tryAction("setVariant", (n) => n.id, true)^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^      : tryAction("setFromString")^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ),^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  "ctrl-d": warnOnError(^\strut\UseVerb{Verb}\SaveVerb{Verb}^tryDeleteChild^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^),^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  "ctrl-c": warnOnError(^\strut\UseVerb{Verb}\SaveVerb{Verb}^() => copyNode(node)^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^),^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  "ctrl-p": warnOnError(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    ^\strut\UseVerb{Verb}\SaveVerb{Verb}^tryAction("replace", (n) => n.id)^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ),^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  "ctrl-f": warnOnError(^\strut\UseVerb{Verb}\SaveVerb{Verb}^editFlags^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^),^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  "ctrl-4": warnOnError(^\strut\UseVerb{Verb}\SaveVerb{Verb}^() =>^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    setMarks({^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^      ...marks,^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^      TODO: idPathFromParentIndexEntry(^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^        parentIndexEntry,^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^      ),^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    })^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ),^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^};^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^for (const [k, v] of handlers) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  handlers[k] = warnOnError(v);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^}^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{a}\\
Type \SaveVerb{Verb}^warnOnError(x)^\adjustbox{bgcolor={HTML}{F2F2F2}}{\strut\UseVerb{Verb}}\\
\keys{\esc}\hspace{2mm}\keys{(}\hspace{2mm}\keys{p}
    \end{flushleft}
  

==> examples/wrap-handlers-4.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^export const handlers = {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  "ctrl-v": warnOnError(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    node.actions.setVariant^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^      ? tryAction("setVariant", (n) => n.id, true)^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^      : tryAction("setFromString"),^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ),^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  "ctrl-d": warnOnError(tryDeleteChild),^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  "ctrl-c": warnOnError(() => copyNode(node)),^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  "ctrl-p": warnOnError(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    tryAction("replace", (n) => n.id),^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ),^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  "ctrl-f": warnOnError(editFlags),^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  "ctrl-4": warnOnError(() =>^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    setMarks({^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^      ...marks,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^      TODO: idPathFromParentIndexEntry(^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^        parentIndexEntry,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^      ),^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^    }),^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ),^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  ^\strut\UseVerb{Verb}\SaveVerb{Verb}^"ctrl-x": ignoreError(cut)^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^,^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^};^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^for (const [k, v] of handlers) {^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^  handlers[k] = warnOnError(v);^\strut\UseVerb{Verb}\\
\SaveVerb{Verb}^}^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{\shift+s}\hspace{2mm}\keys{\arrowkeyright}\hspace{2mm}\keys{\shift+\arrowkeyleft}\hspace{2mm}\keys{\arrowkeyup}\hspace{2mm}\keys{a}\\
Type \SaveVerb{Verb}^,"ctrl-x": ignoreError(cut)^\adjustbox{bgcolor={HTML}{F2F2F2}}{\strut\UseVerb{Verb}}\\
\keys{\esc}
    \end{flushleft}
  

==> examples/wrap-handlers-5.tex <==

    \adjustbox{bgcolor={HTML}{F2F2F2}}{
      \begin{minipage}{\columnwidth}
        \begin{flushleft}
          \setlength{\fboxsep}{0pt}
          \SaveVerb{Verb}^export const handlers = {^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  "ctrl-v": warnOnError(^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    node.actions.setVariant^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^      ? tryAction("setVariant", (n) => n.id, true)^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^      : tryAction("setFromString"),^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  ),^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  "ctrl-d": warnOnError(tryDeleteChild),^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  "ctrl-c": warnOnError(() => copyNode(node)),^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  "ctrl-p": warnOnError(^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    tryAction("replace", (n) => n.id),^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  ),^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  "ctrl-f": warnOnError(editFlags),^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  "ctrl-4": warnOnError(() =>^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    setMarks({^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^      ...marks,^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^      TODO: idPathFromParentIndexEntry(^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^        parentIndexEntry,^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^      ),^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^    }),^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  ),^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^  "ctrl-x": ignoreError(cut),^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\\
\SaveVerb{Verb}^}^\adjustbox{bgcolor={HTML}{A5BFFF}}{\strut\UseVerb{Verb}}\SaveVerb{Verb}^;^\strut\UseVerb{Verb}
        \end{flushleft}
      \end{minipage}
    }
    \begin{flushleft}
      \keys{\}}\hspace{2mm}\keys{\shift+\arrowkeyright}\hspace{2mm}\keys{\SPACE}\hspace{2mm}\keys{d}
    \end{flushleft}
  

==> examples/wrap-handlers.tex <==

\FloatBarrier
\subsection{wrap-handlers}
\label{example:wrap-handlers}
\setcounter{figure}{0}

      \begin{examplestep}
        \small
        \input{examples/wrap-handlers-0.tex}
        \normalsize
        \captionof{figure}{Initial state}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/wrap-handlers-1.tex}
        \normalsize
        \captionof{figure}{Select all properties and split cursor (cursor per property)}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/wrap-handlers-2.tex}
        \normalsize
        \captionof{figure}{Select, copy and delete property value.}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/wrap-handlers-3.tex}
        \normalsize
        \captionof{figure}{Add call to ``warnOnError'' and paste old property value inside.}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/wrap-handlers-4.tex}
        \normalsize
        \captionof{figure}{Remove all cursors except the last and add a new property.}
        
      \end{examplestep}
    

      \begin{examplestep}
        \small
        \input{examples/wrap-handlers-5.tex}
        \normalsize
        \captionof{figure}{Delete the loop that would wrap each property.}
        
      \end{examplestep}
    
\FloatBarrier
  

==> manual-examples/245877a7b73dd3b81d63fe382c23f3eb17c79b31.tex <==
\SaveVerb{Old0}^      } else if (ev.key === "l" && !hasAltLike(ev)) {^
\SaveVerb{Old1}^        const result = cursorMoveLeaf({^
\SaveVerb{Old2}^          root: this.doc.root,^
\SaveVerb{Old3}^          cursor: this.getCursor(),^
\SaveVerb{Old4}^          direction: 1,^
\SaveVerb{Old5}^          extend: false,^
\SaveVerb{Old6}^        });^
\SaveVerb{Old7}^        this.setFromCursor(result.cursor);^
\SaveVerb{Old8}^      } else if (ev.key === "L" && !ev.ctrlKey) {^
\SaveVerb{Old9}^        const result = cursorMoveLeaf({^
\SaveVerb{Old10}^          root: this.doc.root,^
\SaveVerb{Old11}^          cursor: this.getCursor(),^
\SaveVerb{Old12}^          direction: 1,^
\SaveVerb{Old13}^          extend: true,^
\SaveVerb{Old14}^        });^
\SaveVerb{Old15}^        this.setFromCursor(result.cursor);^
\SaveVerb{Old16}^        this.nextEnableReduceToTip = true;^
\SaveVerb{Old17}^      } else if (ev.key === "h" && !hasAltLike(ev)) {^
\SaveVerb{Old18}^        const result = cursorMoveLeaf({^
\SaveVerb{Old19}^          root: this.doc.root,^
\SaveVerb{Old20}^          cursor: this.getCursor(),^
\SaveVerb{Old21}^          direction: -1,^
\SaveVerb{Old22}^          extend: false,^
\SaveVerb{Old23}^        });^
\SaveVerb{Old24}^        this.setFromCursor(result.cursor)^

\SaveVerb{New0}^      } else if (ev.key === "l" && !hasAltLike(ev)) {^
\SaveVerb{New1}^        const result = cursorMoveLeaf({^
\SaveVerb{New2}^          root: this.doc.root,^
\SaveVerb{New3}^          cursor: this.getCursor(),^
\SaveVerb{New4}^          direction: 1,^
\SaveVerb{New5}^          mode: CursorMoveLeafMode.Move,^
\SaveVerb{New6}^        });^
\SaveVerb{New7}^        this.setFromCursor(result.cursor);^
\SaveVerb{New8}^      } else if (ev.key === "L" && !ev.ctrlKey) {^
\SaveVerb{New9}^        const result = cursorMoveLeaf({^
\SaveVerb{New10}^          root: this.doc.root,^
\SaveVerb{New11}^          cursor: this.getCursor(),^
\SaveVerb{New12}^          direction: 1,^
\SaveVerb{New13}^          mode: CursorMoveLeafMode.ExtendSelection,^
\SaveVerb{New14}^        });^
\SaveVerb{New15}^        this.setFromCursor(result.cursor);^
\SaveVerb{New16}^        this.nextEnableReduceToTip = true;^
\SaveVerb{New17}^      } else if (ev.key === "h" && !hasAltLike(ev)) {^
\SaveVerb{New18}^        const result = cursorMoveLeaf({^
\SaveVerb{New19}^          root: this.doc.root,^
\SaveVerb{New20}^          cursor: this.getCursor(),^
\SaveVerb{New21}^          direction: -1,^
\SaveVerb{New22}^          mode: CursorMoveLeafMode.Move,^
\SaveVerb{New23}^        });^
\SaveVerb{New24}^        this.setFromCursor(result.cursor);^

\diffwhole{245877a7b73dd3b81d63fe382c23f3eb17c79b31}{
    \diffomit
    \diffsame{Old0}
    \diffsame{Old1}
    \diffsame{Old2}
    \diffsame{Old3}
    \diffsame{Old4}
    \diffremove{Old5}
    \diffsame{Old6}
    \diffsame{Old7}
    \diffsame{Old8}
    \diffsame{Old9}
    \diffsame{Old10}
    \diffsame{Old11}
    \diffsame{Old12}
    \diffremove{Old13}
    \diffsame{Old14}
    \diffsame{Old15}
    \diffsame{Old16}
    \diffsame{Old17}
    \diffsame{Old18}
    \diffsame{Old19}
    \diffsame{Old20}
    \diffsame{Old21}
    \diffremove{Old22}
    \diffsame{Old23}
    \diffsame{Old24}
    \diffomit
}{
    \diffomit
    \diffsame{New0}
    \diffsame{New1}
    \diffsame{New2}
    \diffsame{New3}
    \diffsame{New4}
    \diffadd{New5}
    \diffsame{New6}
    \diffsame{New7}
    \diffsame{New8}
    \diffsame{New9}
    \diffsame{New10}
    \diffsame{New11}
    \diffsame{New12}
    \diffadd{New13}
    \diffsame{New14}
    \diffsame{New15}
    \diffsame{New16}
    \diffsame{New17}
    \diffsame{New18}
    \diffsame{New19}
    \diffsame{New20}
    \diffsame{New21}
    \diffadd{New22}
    \diffsame{New23}
    \diffsame{New24}
    \diffomit
}{A diff for the simplest edit in the ``specialized edit'' category (Section \ref{sec:evaluation-manual-edits}). The ``extend'' option was replaced by a ``mode'' option, with the boolean value changed to a corresponding enum value. This diff only shows 3 of the 4 edited locations. See \href{https://github.com/tehwalris/forest/commit/245877a7b73dd3b81d63fe382c23f3eb17c79b31}{Forest commit 245877a} for all changes.}


==> manual-examples/44df2e6ba178b33e075e554565a615216338f476.tex <==
\SaveVerb{Old0}^  buildDoc: withExtendedArgsList(^
\SaveVerb{Old1}^    ({ nodeForDisplay, childDocs, newTextNode, updatePostLayoutHints }) => {^
\SaveVerb{Old2}^      updatePostLayoutHints(nodeForDisplay.id, (oldHints) => ({^
\SaveVerb{Old3}^        ...oldHints,^
\SaveVerb{Old4}^        styleAsText: true,^
\SaveVerb{Old5}^      }));^
\SaveVerb{Old6}^      return groupDoc(^
\SaveVerb{Old7}^        childDocs.map((c, i) =>^
\SaveVerb{Old8}^          i === 0^
\SaveVerb{Old9}^            ? c^
\SaveVerb{Old10}^            : groupDoc([^
\SaveVerb{Old11}^                leafDoc(newTextNode(", ", LabelStyle.SYNTAX_SYMBOL)),^
\SaveVerb{Old12}^                c,^
\SaveVerb{Old13}^              ]),^
\SaveVerb{Old14}^        ),^
\SaveVerb{Old15}^      );^
\SaveVerb{Old16}^    },^
\SaveVerb{Old17}^  ),^
\SaveVerb{Old18}^  buildDoc: withExtendedArgsStruct(^
\SaveVerb{Old19}^    ["dotDotDotToken", "name", "questionToken", "type", "initializer"],^
\SaveVerb{Old20}^    ({^
\SaveVerb{Old21}^      nodeForDisplay,^
\SaveVerb{Old22}^      updatePostLayoutHints,^
\SaveVerb{Old23}^      shouldHideChild,^
\SaveVerb{Old24}^      childDocs,^
\SaveVerb{Old25}^      showChildNavigationHints,^
\SaveVerb{Old26}^      newTextNode,^
\SaveVerb{Old27}^    }) => {^
\SaveVerb{Old28}^      if (showChildNavigationHints) {^
\SaveVerb{Old29}^        return undefined;^
\SaveVerb{Old30}^      }^
\SaveVerb{Old31}^      updatePostLayoutHints(nodeForDisplay.id, (oldHints) => ({^
\SaveVerb{Old32}^        ...oldHints,^
\SaveVerb{Old33}^        styleAsText: true,^
\SaveVerb{Old34}^        label: [],^
\SaveVerb{Old35}^      }));^
\SaveVerb{Old36}^      return groupDoc(^
\SaveVerb{Old37}^        filterTruthyChildren([^
\SaveVerb{Old38}^          !shouldHideChild("dotDotDotToken") && childDocs.dotDotDotToken,^
\SaveVerb{Old39}^          childDocs.name,^
\SaveVerb{Old40}^          !shouldHideChild("questionToken") && childDocs.questionToken,^
\SaveVerb{Old41}^          !shouldHideChild("type") && typeWithColon,^
\SaveVerb{Old42}^          !shouldHideChild("initializer") && initializerWithEqualsSign,^
\SaveVerb{Old43}^        ]),^
\SaveVerb{Old44}^      );^
\SaveVerb{Old45}^    },^
\SaveVerb{Old46}^  ),^

\SaveVerb{New0}^  buildDoc: withExtendedArgsList(^
\SaveVerb{New1}^    ({ childDocs, newTextNode, newFocusMarker }) => {^
\SaveVerb{New2}^      return groupDoc([^
\SaveVerb{New3}^        newFocusMarker(),^
\SaveVerb{New4}^        ...childDocs.map((c, i) =>^
\SaveVerb{New5}^          groupDoc([^
\SaveVerb{New6}^            c,^
\SaveVerb{New7}^            leafDoc(newTextNode(",", LabelStyle.SYNTAX_SYMBOL)),^
\SaveVerb{New8}^            lineDoc(),^
\SaveVerb{New9}^          ]),^
\SaveVerb{New10}^        ),^
\SaveVerb{New11}^      ]);^
\SaveVerb{New12}^    },^
\SaveVerb{New13}^  ),^
\SaveVerb{New14}^  buildDoc: withExtendedArgsStruct(^
\SaveVerb{New15}^    ["dotDotDotToken", "name", "questionToken", "type", "initializer"],^
\SaveVerb{New16}^    ({^
\SaveVerb{New17}^      shouldHideChild,^
\SaveVerb{New18}^      childDocs,^
\SaveVerb{New19}^      showChildNavigationHints,^
\SaveVerb{New20}^      newTextNode,^
\SaveVerb{New21}^      newFocusMarker,^
\SaveVerb{New22}^    }) => {^
\SaveVerb{New23}^      if (showChildNavigationHints) {^
\SaveVerb{New24}^        return undefined;^
\SaveVerb{New25}^      }^
\SaveVerb{New26}^      const initializerWithEqualsSign = groupDoc([^
\SaveVerb{New27}^        leafDoc(newTextNode(" = ", LabelStyle.SYNTAX_SYMBOL)),^
\SaveVerb{New28}^        childDocs.initializer,^
\SaveVerb{New29}^      ]);^
\SaveVerb{New30}^      const typeWithColon: Doc = groupDoc([^
\SaveVerb{New31}^        leafDoc(newTextNode(": ", LabelStyle.SYNTAX_SYMBOL)),^
\SaveVerb{New32}^        childDocs.type,^
\SaveVerb{New33}^      ]);^
\SaveVerb{New34}^      return groupDoc(^
\SaveVerb{New35}^        filterTruthyChildren([^
\SaveVerb{New36}^          newFocusMarker(),^
\SaveVerb{New37}^          !shouldHideChild("dotDotDotToken") && childDocs.dotDotDotToken,^
\SaveVerb{New38}^          childDocs.name,^
\SaveVerb{New39}^          !shouldHideChild("questionToken") && childDocs.questionToken,^
\SaveVerb{New40}^          !shouldHideChild("type") && typeWithColon,^
\SaveVerb{New41}^          !shouldHideChild("initializer") && initializerWithEqualsSign,^
\SaveVerb{New42}^        ]),^
\SaveVerb{New43}^      );^
\SaveVerb{New44}^    },^
\SaveVerb{New45}^  ),^

\diffwholespecial{44df2e6ba178b33e075e554565a615216338f476}{
    \diffomit
    \diffsame{Old0}
    \diffremove{Old1}
    \diffadd{New1}
    \diffremove{Old2}
    \diffremove{Old3}
    \diffremove{Old4}
    \diffremove{Old5}
    \diffremove{Old6}
    \diffadd{New2}
    \diffadd{New3}
    \diffremove{Old7}
    \diffadd{New4}
    \diffsame{Old8}
    \diffsame{Old9}
    \diffsame{Old10}
    \diffsame{Old11}
    \diffsame{Old12}
    \diffsame{Old13}
    \diffsame{Old14}
    \diffremove{Old15}
    \diffadd{New11}
    \diffsame{Old16}
    \diffsame{Old17}
    \diffomit
}{A diff for the most complex edit in the ``specialized edit'' category (Section \ref{sec:evaluation-manual-edits}). Calls to  ``updatePostLayoutHints'' within a ``buildDoc'' method are removed. Instead, a call to ``newFocusMarker'' is added to the an array literal in the returned ``groupDoc'' call. If ``groupDoc'' does not contain an array literal, it is created and the old content is spread. Required/unused arguments are added to the ``withExtendedArgsList'' and ``withExtendedArgsStruct'' calls as needed. This diff only shows 1 of the 5 edited locations. A second edited location is shown in Figure \ref{fig:44df2e6ba178b33e075e554565a615216338f476-second}. See \href{https://github.com/tehwalris/forest/commit/44df2e6ba178b33e075e554565a615216338f476}{Forest commit 44df2e6} for all changes.}{
    \diffomit
    \diffsame{Old18}
    \diffsame{Old19}
    \diffsame{Old20}
    \diffremove{Old21}
    \diffremove{Old22}
    \diffsame{Old23}
    \diffsame{Old24}
    \diffsame{Old25}
    \diffsame{Old26}
    \diffadd{New21}
    \diffsame{Old27}
    \diffsame{Old28}
    \diffsame{Old29}
    \diffsame{Old30}
    \diffremove{Old31}
    \diffremove{Old32}
    \diffremove{Old33}
    \diffremove{Old34}
    \diffremove{Old35}
    \diffomit
    \diffsame{Old36}
    \diffsame{Old37}
    \diffadd{New36}
    \diffsame{Old38}
    \diffsame{Old39}
    \diffsame{Old40}
    \diffsame{Old41}
    \diffsame{Old42}
    \diffsame{Old43}
    \diffsame{Old44}
    \diffsame{Old45}
    \diffsame{Old46}
    \diffomit
}{The second edited location described in Figure \ref{fig:44df2e6ba178b33e075e554565a615216338f476-first}.}

==> manual-examples/8d8ac11f5d8faae6868d7a003beb7b04eeea5ed0.tex <==
\SaveVerb{Old0}^     } else if (ev.key === "k") {^
\SaveVerb{Old1}^      this.cursors = this.cursors.map(^
\SaveVerb{Old2}^        (cursor) =>^
\SaveVerb{Old3}^          cursorMoveInOut({^
\SaveVerb{Old4}^            root: this.doc.root,^
\SaveVerb{Old5}^            cursor: cursor,^
\SaveVerb{Old6}^            direction: CursorMoveInOutDirection.Out,^
\SaveVerb{Old7}^            bigStep: false,^
\SaveVerb{Old8}^          }).cursor,^
\SaveVerb{Old9}^      );^
\SaveVerb{Old10}^    } else if (ev.key === "K") {^
\SaveVerb{Old11}^    } else if ([")", "]", "}", ">"].includes(ev.key)) {^
\SaveVerb{Old12}^      this.cursors = this.cursors.map(^
\SaveVerb{Old13}^        (cursor) =>^
\SaveVerb{Old14}^          cursorMoveInOut({^
\SaveVerb{Old15}^            root: this.doc.root,^
\SaveVerb{Old16}^            cursor: cursor,^
\SaveVerb{Old17}^            direction: CursorMoveInOutDirection.Out,^
\SaveVerb{Old18}^            bigStep: true,^
\SaveVerb{Old19}^            delimiter: ev.key,^
\SaveVerb{Old20}^          }).cursor,^
\SaveVerb{Old21}^      );^

\SaveVerb{New0}^    } else if (ev.key === "k") {^
\SaveVerb{New1}^      this.multiCursorHelper(^
\SaveVerb{New2}^        (strict) =>^
\SaveVerb{New3}^          multiCursorMoveInOut({^
\SaveVerb{New4}^            root: this.doc.root,^
\SaveVerb{New5}^            cursors: this.cursors,^
\SaveVerb{New6}^            direction: CursorMoveInOutDirection.Out,^
\SaveVerb{New7}^            bigStep: false,^
\SaveVerb{New8}^            strict,^
\SaveVerb{New9}^          }),^
\SaveVerb{New10}^        (result) => {^
\SaveVerb{New11}^          this.cursors = result.cursors;^
\SaveVerb{New12}^        },^
\SaveVerb{New13}^      );^
\SaveVerb{New14}^    } else if (ev.key === "K") {^
\SaveVerb{New15}^    } else if ([")", "]", "}", ">"].includes(ev.key)) {^
\SaveVerb{New16}^      this.multiCursorHelper(^
\SaveVerb{New17}^        (strict) =>^
\SaveVerb{New18}^          multiCursorMoveInOut({^
\SaveVerb{New19}^            root: this.doc.root,^
\SaveVerb{New20}^            cursors: this.cursors,^
\SaveVerb{New21}^            direction: CursorMoveInOutDirection.Out,^
\SaveVerb{New22}^            bigStep: true,^
\SaveVerb{New23}^            delimiter: ev.key,^
\SaveVerb{New24}^            strict,^
\SaveVerb{New25}^          }),^
\SaveVerb{New26}^        (result) => {^
\SaveVerb{New27}^          this.cursors = result.cursors;^
\SaveVerb{New28}^        },^
\SaveVerb{New29}^      );^

\diffwhole{8d8ac11f5d8faae6868d7a003beb7b04eeea5ed0}{
    \diffomit
    \diffsame{Old0}
    \diffremove{Old1}
    \diffremove{Old2}
    \diffremove{Old3}
    \diffsame{Old4}
    \diffremove{Old5}
    \diffsame{Old6}
    \diffsame{Old7}
    \diffalign
    \diffremove{Old8}
    \diffalign
    \diffalign
    \diffalign
    \diffsame{Old9}
    \diffsame{Old10}
    \diffomit
    \diffsame{Old11}
    \diffremove{Old12}
    \diffremove{Old13}
    \diffremove{Old14}
    \diffsame{Old15}
    \diffremove{Old16}
    \diffsame{Old17}
    \diffsame{Old18}
    \diffsame{Old19}
    \diffalign
    \diffremove{Old20}
    \diffalign
    \diffalign
    \diffalign
    \diffsame{Old21}
    \diffomit
}{
    \diffomit
    \diffsame{New0}
    \diffadd{New1}
    \diffadd{New2}
    \diffadd{New3}
    \diffsame{New4}
    \diffadd{New5}
    \diffsame{New6}
    \diffsame{New7}
    \diffadd{New8}
    \diffadd{New9}
    \diffadd{New10}
    \diffadd{New11}
    \diffadd{New12}
    \diffsame{New13}
    \diffsame{New14}
    \diffomit
    \diffsame{New15}
    \diffadd{New16}
    \diffadd{New17}
    \diffadd{New18}
    \diffsame{New19}
    \diffadd{New20}
    \diffsame{New21}
    \diffsame{New22}
    \diffsame{New23}
    \diffadd{New24}
    \diffadd{New25}
    \diffadd{New26}
    \diffadd{New27}
    \diffadd{New28}
    \diffsame{New29}
    \diffomit
}{A diff for an edit of slightly above average complexity in the ``specialized edit'' category (Section \ref{sec:evaluation-manual-edits}). Instead of handling cursors directly using ``this.cursors.map'', the helper function ``multiCursorHelper'' is introduced. The passing of the ``cursors'' argument and the handling of the return value changes accordingly. Additionally a new ``strict'' option must be forwarded. This diff only shows 2 of the 5 edited locations. See \href{https://github.com/tehwalris/forest/commit/8d8ac11f5d8faae6868d7a003beb7b04eeea5ed0}{Forest commit 8d8ac11} for all changes.}

==> manual-examples/index.tex <==
\input{manual-examples/245877a7b73dd3b81d63fe382c23f3eb17c79b31}\clearpage
\input{manual-examples/8d8ac11f5d8faae6868d7a003beb7b04eeea5ed0}\clearpage
\input{manual-examples/44df2e6ba178b33e075e554565a615216338f476}\clearpage

==> manual-examples/wrap-handlers-diff.tex <==
\SaveVerb{Old0}^export const handlers = {^
\SaveVerb{Old1}^  "ctrl-v": node.actions.setVariant^
\SaveVerb{Old2}^    ? tryAction("setVariant", n => n.id, true)^
\SaveVerb{Old3}^    : tryAction("setFromString"),^
\SaveVerb{Old4}^  "ctrl-d": tryDeleteChild,^
\SaveVerb{Old5}^  "ctrl-c": () => copyNode(node),^
\SaveVerb{Old6}^  "ctrl-p": tryAction("replace", n => n.id),^
\SaveVerb{Old7}^  "ctrl-f": editFlags,^
\SaveVerb{Old8}^  "ctrl-4": () =>^
\SaveVerb{Old9}^    setMarks({ ...marks, TODO: f(parentIndexEntry) }),^
\SaveVerb{Old10}^};^
\SaveVerb{Old11}^for (const [k, v] of handlers) {^
\SaveVerb{Old12}^  handlers[k] = warnOnError(v);^
\SaveVerb{Old13}^}^

\SaveVerb{New0}^export const handlers = {^
\SaveVerb{New1}^  "ctrl-v": warnOnError(^
\SaveVerb{New2}^    node.actions.setVariant^
\SaveVerb{New3}^      ? tryAction("setVariant", n => n.id, true)^
\SaveVerb{New4}^      : tryAction("setFromString"),^
\SaveVerb{New5}^  ),^
\SaveVerb{New6}^  "ctrl-d": warnOnError(tryDeleteChild),^
\SaveVerb{New7}^  "ctrl-c": warnOnError(() => copyNode(node)),^
\SaveVerb{New8}^  "ctrl-p": warnOnError(tryAction("replace", n => n.id)),^
\SaveVerb{New9}^  "ctrl-f": warnOnError(editFlags),^
\SaveVerb{New10}^  "ctrl-4": warnOnError(() =>^
\SaveVerb{New11}^    setMarks({ ...marks, TODO: f(parentIndexEntry) }),^
\SaveVerb{New12}^  ),^
\SaveVerb{New13}^  "ctrl-x": ignoreError(cut),^
\SaveVerb{New14}^};^

\diffbody{
    \diffsame{Old0}
    \diffremove{Old1}
    \diffalign
    \diffsame{Old2}
    \diffsame{Old3}
    \diffalign
    \diffremove{Old4}
    \diffremove{Old5}
    \diffremove{Old6}
    \diffremove{Old7}
    \diffremove{Old8}
    \diffsame{Old9}
    \diffalign
    \diffalign
    \diffsame{Old10}
    \diffremove{Old11}
    \diffremove{Old12}
    \diffremove{Old13}
}{
    \diffsame{New0}
    \diffadd{New1}
    \diffadd{New2}
    \diffsame{New3}
    \diffsame{New4}
    \diffadd{New5}
    \diffadd{New6}
    \diffadd{New7}
    \diffadd{New8}
    \diffadd{New9}
    \diffadd{New10}
    \diffsame{New11}
    \diffadd{New12}
    \diffadd{New13}
    \diffsame{New14}
    \diffalign
    \diffalign
    \diffalign
}

==> sections/evaluation-manual-edits.tex <==
Refactoring scripts are generally used to perform large-scale edits which would be impractical with manual editing. In some situations, a developer needs to make a similar change in multiple locations, but too few to justify writing a refactoring script. A multi-cursor editor could be used to potentially perform such edits more efficiently than manual single-cursor editing. To understand whether the small-scale edits that occur in real TypeScript codebases could be performed effectively with a multi-cursor editor, we manually inspected all of the commits in Forest's codebase and classified the kinds of edits that were performed.

\subsection{Method}
We manually inspected every commit in Forest's codebase to identify edits which a multi-cursor editor could potentially perform effectively. We then more closely analyzed a subset of the commits which had potential for multi-cursor editing.

\paragraph{Initial Classification} Forest's codebase contained 913 commits at the time of our evaluation. There are roughly 5-20 commits per full workday, so most commits were small enough that individual edits were clearly visible in their diffs. We manually classified each commit based on whether it would potentially be useful to perform part of its edit with a multi-cursor editor: 

\begin{itemize}
    \item \emph{No}: The commit contains no edits that a multi-cursor editor could perform especially effectively.
    \item \emph{Yes}: Some edit in the commit could potentially be performed effectively using multiple cursors in a multi-cursor editor.
\end{itemize}

\paragraph{Classification Guidelines} Estimating \emph{potential for effective multi-cursor editing} is subjective. We looked for patterns such as multiple insertions or changes that appeared similar. We considered whether a \emph{hypothetical} multi-cursor editor could simultaneously edit these locations. We based this on our experience with existing multi-cursor editors (Kakoune for text and Forest for structure) and considered whether a similar editor (potentially with added features) could perform the edit. When in doubt, we classified commits as \emph{Yes}, to avoid discarding potentially interesting commits before the next stage of our evaluation.

\paragraph{Ignoring Renames} Importantly, we classified edits that could be performed using a ``rename identifier'' refactor in a standard IDE as \emph{No}. This refactor was commonly used in the Forest codebase and always performed the desired edits perfectly. We think that there is no room for multi-cursor editors to improve this result. However, multi-cursor editors could include the same refactor that is used in existing IDEs, so they are not at a disadvantage either.

\paragraph{Further Classification} We further investigated the commits which were classified \emph{Yes} in the previous evaluation stage. Due to time constraints, we only considered a random sample of 50\% of those commits. For each commit, we grouped the changes (excluding those where multi-cursor editing would not be useful) into multiple \emph{edits}. Each edit would be performed simultaneously using multiple cursors. For each edit, we tried to describe the type of edit that was performed and estimated the number of cursors that the edit would use.

\subsection{Results}
\label{sec:results-manual-edits}
In our initial classification stage, we classified 142 of 913 commits (\mytilde{}15\%) \emph{Yes}, meaning that they contained edits that could potentially be performed effectively using multiple cursors in a multi-cursor editor. We further investigated a random sample of 50\% (71) of the 142 \emph{Yes} commits. The number of distinct edits with multi-cursor potential per commit is shown in Figure \ref{fig:edits-per-commit}. Most commits contained one such edit. Although all commits were assigned \emph{Yes} in the initial classification, closer inspection during further classification revealed that 10 commits contained no edits that we believe could plausibly be performed with a multi-cursor editor. These edits typically changed multiple similar locations, but inserted varied content in each one. Most edits used a small number of cursors (2--5) as shown in Figure \ref{fig:cursors-per-edit}. Table \ref{table:edit-categories} shows the types of edits that we found. In the rest of this section, we describe the most common types of edits in detail.

\begin{figure}[h]
\includegraphics[width=\columnwidth]{plots/edits-per-commit.pdf}
\caption{Number of edits with multi-cursor potential in each commit}
\label{fig:edits-per-commit}
\end{figure}

\begin{figure}[h]
\includegraphics[width=\columnwidth]{plots/cursors-per-edit.pdf}
\caption{Estimated number of cursors required for each edit with multi-cursor potential}
\label{fig:cursors-per-edit}
\end{figure}

\begin{table}[ht]
\begin{tabular}{@{}cl@{}} \toprule
Count & Category \\\midrule
22 & specialized edit \\
17 & rename-like replace \\
16 & add/remove required argument/property \\
11 & wrap expression/statement \\
6 & identical insertion \\
4 & insertion with small unique part \\
4 & delete a declaration and everything related \\
3 & extract expression into function/variable \\
2 & add/remove modifier \\
2 & add destructure, type and value \\
1 & flatten variable declarations \\
\bottomrule
\vspace{0.1cm}
\end{tabular}
\caption{Categories of edits with potential for multi-cursor editing from commits in the codebase of Forest.}
\label{table:edit-categories}
\end{table}

\paragraph{``specialized edit''}
This category contains edits that do not fit in any other categories. These edits were generally simple structural transformations, but ones that are specific to the program being edited. To give an intuition of the kinds of edits in this category, we provide some examples: Figure \ref{fig:245877a7b73dd3b81d63fe382c23f3eb17c79b31} (Example \ref{example:245877a7b73dd3b81d63fe382c23f3eb17c79b31}) shows the simplest edit in this category, where booleans are replaced by one of two enum values. Figure \ref{fig:8d8ac11f5d8faae6868d7a003beb7b04eeea5ed0} (Example \ref{example:8d8ac11f5d8faae6868d7a003beb7b04eeea5ed0}) shows an edit of slightly above average complexity, where one function call is replaced by another, which requires introducing new arguments and changing the handling of return values. Figures \ref{fig:44df2e6ba178b33e075e554565a615216338f476-first} and \ref{fig:44df2e6ba178b33e075e554565a615216338f476-second} (Example \ref{example:44df2e6ba178b33e075e554565a615216338f476}) show the most complex edit in this category, where a function call is removed and a new call is inserted in the nearest array literal, which requires various related adjustments to the code.

% not belong to another category are grouped here. \todo[inline]{write more}

\paragraph{``rename-like replace''}
In such an edit, every usage of a variable, class property, or object field was replaced by a new expression. For example, consider a class with the properties \lstinline{cursors: Cursor[]} and \lstinline{oldCursors: Cursor[]} (accessed via \lstinline{this.cursors} and \lstinline{this.oldCursors}). If the developer replaces all usages (potentially within a limited area) of \linebreak\lstinline{this.oldCursors} by usages of \lstinline{this.cursors}, that would be a rename-like replace. The defining feature of this edit is that it affects the same locations as renaming the \lstinline{oldCursors} property affects, except that the property declaration itself is not changed (only the usages are replaced). An additional difference to a typical rename is that target locations can be replaced by any expression, not just the same one with a new identifier (e.g., \lstinline{this.oldCursors} could be replaced by \lstinline{this.oldState.cursors}). If the new expression differs at each replacement location (e.g., it wraps the old expression), the edit is counted as a \emph{specialized edit}.

\paragraph{``add/remove required argument/property''}
When a required parameter is added to a function declaration, an appropriate expression must be added to the argument list at every call site to fix type errors. Similar edits must be performed when a required argument is removed, or when an interface property is added or removed. This category captures such edits, but only those where the added argument expression is the same at every call site. If the added argument differs at each call site (e.g., is copied from near the call), the edit is counted as a \emph{specialized edit}.

\paragraph{``wrap expression/statement''}
In such an edit, an expression (e.g., \lstinline{getInput()}) is replaced by an expression which contains the original somewhere inside (for example, \linebreak\lstinline${ device: 'keyboard', input: getInput() }$). If the original expression appears more than once in the replacement, or if any part of the original expression is modified (e.g., adding an argument to \lstinline{getInput()}), then the edit is counted as a \emph{specialized edit}.

\paragraph{``identical insertion''}
In such an edit, the same code is inserted in multiple locations. The inserted code does not wrap or replace any existing code. If any part of the inserted code varies, then the edit is counted as \emph{insertion with small unique part}.

\paragraph{``insertion with small unique part''}
In such an edit, nearly the same code is inserted in multiple locations, but a small part of the inserted code differs. For example, a large object literal with boilerplate values is inserted in multiple locations, and then a single property value is changed at each location. The differing part is typically hard to systematically guess, requiring a deep understanding of the code.

\paragraph{``delete a declaration and everything related''}
When a declaration (e.g., an enum declaration) is deleted, the user often also deletes related code (e.g., every interface declaration or function argument where the deleted enum was used). The extent of the deletion varies and generally has to be decided by the user (e.g., should the properties of an interface which have the type of the deleted enum type be deleted, or should the whole interface declaration be deleted?). 

\paragraph{``extract expression into function/variable''}
In such an edit, multiple copies of an identical expression are replaced by references to a newly created variable containing the expression. If part of the expression varies at each usage site, the common part of the expression could be expected into a function.

\paragraph{``add/remove modifier''}
In such an edit, modifiers (e.g \lstinline{public}, \lstinline{async}, \lstinline{export}) are added or removed (e.g., from methods or variable declarations). In our evaluation, this edit was only ever performed by adding or removing the \lstinline{export} keyword from function declarations. 

